Pixel-wise Distance Regression for Glacier Calving Front Detection and Segmentation

Glacier calving front position (CFP) is an important glaciological variable. Traditionally, delineating the CFPs has been carried out manually, which was subjective, tedious and expensive. Automating this process is crucial for continuously monitoring the evolution and status of glaciers. Recently, deep learning approaches have been investigated for this application. However, the current methods get challenged by a severe class-imbalance problem. In this work, we propose to mitigate the class-imbalance between the calving front class and the non-calving front class by reformulating the segmentation problem into a pixel-wise regression task. A Convolutional Neural Network gets optimized to predict the distance values to the glacier front for each pixel in the image. The resulting distance map localizes the CFP and is further post-processed to extract the calving front line. We propose three post-processing methods, one method based on statistical thresholding, a second method based on conditional random fields (CRF), and finally the use of a second U-Net. The experimental results confirm that our approach significantly outperforms the state-of-the-art methods and produces accurate delineation. The Second U-Net obtains the best performance results, resulting in an average improvement of about 21% dice coefficient enhancement.

==> 30_evaluation_old_EnzeModels.tex <==
% !TeX spellcheck = en_US
\begin{figure*}
	\centering
	\includegraphics[width=0.9\linewidth]{Figures/AP-front-overview-2_updated.png}
	\caption{Overview of studied glaciers on the northern Antarctic Peninsula. Pink polygons indicate the subsets used in the analysis. Background: Bing Aerial Maps © Microsoft; Map of Antarctica: Landsat LIMA Mosaic © USGS, NASA, BAS, NFS.}
	\label{fig:front_overview}
\end{figure*}
\section{Evaluation}\label{sec:evaluation}
\subsection{Dataset}\label{sec:dataset}
\subsubsection{Study Sites}
We selected outlet glaciers at the Antarctic Peninsula (AP) %and Greenland 
to train and evaluate the glacier front mapping on SAR intensity imagery using CNN.
The AP is a hot spot of global climate change. A significant temperature increase was reported for the 20th century~\cite{oliva2017recent, turner2016absence} %(e.g. Oliva et al., 2017; Turner et al., 2016)
strongly affecting its ice sheets. Pronounced retreat and even disintegration of the ice shelves along the AP was observed~\cite{cook2010overview}. %(Cook and Vaughan, 2010)
Most of the northern ice shelves at the Prince-Gustav-Channel (PGC) and Larsen-A embayment disintegrated in 1995, and at the Larsen-B embayment in 2002~\cite{cooper1997historical, scambos2004glacier, skvarca1998evidence}. %(Cooper, 1997; Scambos, 2004; Skvarca et al., 1998)
The reduction of the buttressing forces led to a strong increase in ice discharge and further frontal retreat of the former ice shelf tributary glaciers~\cite{rott2014mass, seehaus2015changes}. %(Rott et al., 2014; Seehaus et al., 2015) 
Due to its relevance and the data availability, we selected several of these former ice shelf tributaries for our analysis (see \cref{fig:front_overview}).
%

The glacier system of the Sjögren-Inlet (SI) and Dinsmoore-Bombardier-Edgworth (DBE) glacier systems were major tributaries to the PGC and Larsen-A ice shelves, respectively. Seehaus et al.~\cite{seehaus2015changes, seehaus2016dynamic} %(2015, 2016) 
carried out a detailed analysis of the glacier evolution after the disintegration of the ice shelves. {\color{red}{(TODO: Ambiguous$\rightarrow$Rephrase?) After the disintegration a strong increase in ice discharge, with a subsequent long-term decrease was obtained.}} Simultaneously, the glacier fronts strongly retreated after the ice shelf disintegration and stabilized at SI glacier system after about 15 years, whereas at DBE glacier re-advance and short-term recession were observed.
Crane, Mapple and Jorum glaciers are former tributaries of the Larsen-B ice shelf. Rott et al. reported a similar reaction to the ice shelf break-up as DBE and SI glacier systems~\cite{rott2014mass, tc-12-1273-2018}. %(e.g. Rott et al., 2018, 2014).

%\subsubsection{SAR Imagery Processing}
At the AP, we used imagery from the satellite missions ERS-1/2, Envisat, RadarSAT-1, ALOS, TerraSAR-X (TSX) and TanDEM-X (TDX), covering the period 1995-2014. The German Aerospace Center (DLR), the European Space Agency (ESA) and the Alaska Satellite Facility (ASF) provided the SAR data for our analysis, via granted data proposals. The SAR acquisitions were multilooked to reduce speckle noise and calibrated. The ASTER digital elevation model of the AP~\cite{cook2012new} was used for geocoding and orthorectification of the images. The specifications and parameters of the SAR sensors and imagery are provided in Tab. \ref{tab:sar_sensors}. The GAMMA RS Software was used for processing the imagery.
%
\begin{table*}[hbt]
	\centering
	\begin{tabular}{c c c c c c c c}
		Platform	& Sensor	& Mode	& SAR band	& \makecell{Repetition\\cycle\\{}[d]}	& Time interval	& \makecell{Multi\\looking\\factor}	& \makecell{Ground range\\resolution\\{}[m]} 	\\ \toprule
		Antarctic Peninsula  & & & & & & & 	\\ \midrule
		ERS-1/2	& SAR	& IM	& C band	& 35/1	& \makecell{05. July 1992 -\\ 26. February 2010}	& 1x5	& 20	\\
		\makecell{RADARSAT 1 \\ (SLC \& PRI\\format)}	& SAR	& ST	& C band	& 24	& \makecell{10. September 2000 -\\ 20. January 2008}	& 1x4	& \makecell{20 (SLC) \\ 12.5 (PRI)}	\\
		Envisat	& ASAR	& IM	& C band	& 35	& \makecell{05. December 2003 -\\ 03. July 2010}	& 1x5	& 20	\\[0.3cm]
		ALOS	& PALSAR	& FBS	& L band	& 46	& \makecell{18. May 2006 -\\ 03. March 2011}	& 2x5	& 16,7	\\
		\makecell{TerraSAR-X \\ TanDEM-X \\ (SLC format)}	& SAR	& SM	& X band	& 11	& \makecell{13. October 2008 -\\ 22. December 2014}	& 3x3	& 6.7	\\ \bottomrule
	\end{tabular}
	\caption{Overview of SAR sensors and specifications.}
	\label{tab:sar_sensors}
\end{table*}
%
%We could apply the same preprocessing on the TSX enhanced-ellipsoid-corrected (EEC) data sets that where used by Zhang et al.~\cite{zhang2019automatically} for Jakobshavn Isbrea. The preprocessing algorithms were kindly provided by the authors and get described in detail in Zhang et al.~\cite{zhang2019automatically}.

\subsubsection{Data Generation}
The manually annotated calving front positions for the DBE and SI glacier systems have been generated and used by Seehaus et al.~\cite{seehaus2015changes, seehaus2016dynamic}. Additionally, we manually annotated the glacier front positions of the Larsen-B embayment.
{\color{red}{\\TODO: Talk about the zone and line ground truth and provide an example figure 1x3.\\}}
A quality factor, ranging from $1$ to $6$, was assigned to each SAR image. The quality factors are a subjective measure of the reliability of the picked front position depending on the similarity of the ice mélange and the glacier, with $1$ being the most reliable and $6$ the most unreliable. %Table 1 shows the quality factors and the respective uncertainty values, perpendicular to the glacier front. 
In this study, we discarded the glacier fronts with a quality factor of $6$.
%
\begin{table}[b]
	\centering
	\def\arraystretch{1.5}
	\begin{tabular}{| c ||c |c | c |c |c |c|}
		\hline
		\makecell{Quality  \\ factor}& 1	& 2	& 3	& 4	& 5	& 6	 \\
		\hline
		
		$\sigma_{f}(m)$ & 70 & 130 & 200 & 230 & 450 & - \\
		\hline
	\end{tabular}
	\caption{Quality factors of manual glacier front detection and the assigned horizontal accuracies $\sigma_{f}$ (perpendicular to estimated glacier front position). {\color{red}{TODO: What is the 2nd row? Where in the text should we refer to this table? Current place is not good!}}}
	\label{tab:quality_factors}
\end{table}

%The manually picked glacier fronts generated by Zhang et al. (2019) were used at Jakobshavn Isbrea.
Subsets of the preprocessed SAR intensity imagery were generated covering the areas of interest (see Fig. \ref{fig:front_overview}) and converted to 16-bit single channel images. {\color{red}{(TODO: Ambiguous$\rightarrow$Rephrase?) For each manually picked glacier front position (spatial line) was combined with the coastline and rock-outcrop polygons (based on the Antarctic Digital Database at the AP) to generate a categorized 8bit single channel image.}}
%(four categories: ocean, glacier, rocks and no-data areas in the SAR image) 
The ground truth images have the same size and resolution as the respective SAR image subsets and are used for training the models.

\subsection{Experiments}
First, we compute the distances maps from the glacier front lines (ground truth). We set the decay parameter $\gamma=7$, which produced the best result within the set $\gamma \in \{1\dots10\}$. The same decay value is also used by Meyer et al.~\cite{meyer2018pixel}. The SAR images and the distance maps are then resized to to $512 \times 512$ using linear interpolation.
We train the U-Net from scratch with $310$ training images with batch size of $3$. Because of the limited training set size, we augment the images by flipping and rotating for $90$, $180$, $270$ degrees, which enlarges our training set by the factor of $8$. The training is terminated when the loss value on the validation set, which includes $78$ images, does not decrease for $30$ consecutive epochs. We use the Adam optimizer with a learning rate of $0.001$ to minimize mean squared error (MSE) loss function. The training lasted for $83$ epochs and resulted in validation MSE of $0.003 \pm 0.010$. The model shows visually consistent and accurate distance map prediction results across the validation and test data set. 

%In order to compare the different approaches.
In the next step, we resized the predicted distance map back to the original image size. We use bi-cubic interpolation to implement a smooth transformation with less distortion. From here, we apply the different post processing approaches that we discussed earlier in Sec. \ref{sec:post-processing} to extract the final calving front line. The three different post processing algorithms are parameterized as follows:
%
\subsubsection{Statistical Thresholding} 
We set the percentage of pixels for the threshold value over each image to $95\%$, such that most of lower values from the distance map get removed. This results in a narrow shape mask containing our predicted calving front. {\color{red}{What about the parameters of the morphological thinning, i.e., the structuring element shape and size?}}
	
\subsubsection{Conditional Random Field} 
As for the majority of the parameters' values in the CRF model, we followed Chen et al.~\cite{DBLP:journals/corr/ChenPK0Y16}. {\color{red}{TODO: please mention the parameters and their values here.}} However, we increase the standard deviation of the Bilateral kernel to $\theta_{\alpha}=512$, which overall decreases the amount of artifacts and narrows the spread of the generated glacier front. We also removed the influence of the Gaussian potential, as it further reduced the width of the generated fronts and achieved the most accurate front line.
%could not detect any negative impact.

\subsubsection{Second U-Net}
The model is trained with distance maps predicted by the pixel-wise regression model with the objective of segmenting the calving fronts. We bypass the class-imbalance problem by morphologically dilating the ground truth calving front line with a $5 \times 5$ kernel as the structuring element (SE). The same dataset split is preserved to ensure a comparable evaluation. In the optimization process, we used the Adam optimizer with the learning rate of lr=$5e^{-6}$ to minimize the binary cross-entropy (BCE) loss function. %We train the model to minimize the binary cross entropy (bce) loss function using the Adam optimizer and a learning rate of $5e^{-6}$.
We use the same U-Net architecture and initialize it analogous to the previous model. Using the same early stopping policy as before, the training took $16$ epochs. %Afterwards, we binarize the model output, which determines the calving front affiliation for each pixel.
{\color{red}{TODO: After the first step, you said you resized the results back to the original image size. For the seconds U-Net, what image size did you use? Did you resize to $512\times512$ or did you extracted patches?}}

The individual approaches above show different results. Especially the width of the predicted glacier front lines significantly vary from one approach to another.
To ensure a fair comparison, we adjusted the width of the predictions. 
Since both the CRF and the Second U-Net methods predict thicker glacier fronts, we had to shrink them for the evaluation phase. The output of the Statistical Thresholding method has a single pixel width (skeleton), hence we expand it accordingly. We use the morphological dilation and erosion to adjust the width of the predicted glacier calving front lines. In the width adjustment process, we searched for the optimum structuring element (SE) size resulting in small difference in the sum of calving front pixels for different approaches on a few test images and then applied it to the entire evaluation. 

We compare our results with the calving front line segmentation approach proposed by Zhang et al.~\cite{zhang2019automatically}. {\color{blue}{Here, each image gets subdivide into small patches, which are individually segmented by the U-Net. Afterwards, the patches get merged back to the original image size, which results in the final segmentation output. %We apply the same dataset split that we utilized for our deep learning pipeline. Also in this approach we try to predict the glacier front directly, which differs from the original study by Zhang et al.~\cite{zhang2019automatically}, where the two classes consists of ice mélange and non ice mélange region, rather than calving and non calving front.
The U-Net architecture is trained with the extracted patches using Adam Optimizer and the BCE loss function. The training was stopped by the early stopping mechanism after $64$ epochs.



%%%%%%% NEW	%%%%%%% 

All models share the same architecture, proposed by Zhang et al.~\cite{zhang2019automatically}. Each model is trained using the Adam Optimizer with $\text{lr}=1e-5$. The evaluation loss has been monitored during the training and the training got terminated if the validation loss does not increase for $30$ consecutive epochs.

We train the first model using the {\color{red}{zone masks}} ground truth, which comprise the whole glacier as one class and the ice melange as the other class. We split each image into $512 \times 512$ patches. The training took $103$ epochs. As described by Zhang et al.~\cite{zhang2019automatically}, the method requires some post-processing to extract the glacier fronts. In the first step, the prediction gets binarized to extract the segmented glacier. The prediction includes many artifacts. Therefore, we filled in the small holes and gaps in the predicted segmentation mask using morphological closing and removed the remaining artifacts by extracting the largest connected component. The edge in our labeled segmentation masks defines the glacier front, which was automatically extracted using Canny edge detection algorithm.

The front patch models are both trained using the extracted patches of the dataset. The segmentation mask only includes the glacier front. The front patches model is trained with a patch size of 256x256 and finished training after 63 epochs. The predicted patches get combined and binarized to generate the final calving front. In the front patches model with dilation we widen the glacier front in the segmentation mask of each patch with a 5x5 kernel. Thus we reduce the severe imbalance between the two classes in our segmentation mask. We use patches with a size of 512x512. The training halted after 78 epochs. Like previously we combine the predicted glacier front patches and binarize the output to get the glacier front.

In another approach, we resize the imagery to the model input size of 512x512. With the unified sizes in the dataset we train the model. The training stopped after 89 epochs. As before, we train another model where we also dilate the glacier front mask with 5x5 kernel as structuring element. This model also finished training after 89 epochs. Afterwards we resize the predicted glacier front back to the original image size. We use bi-cubic interpolation to implement a smooth transformation with less distortion. The result gets binarized to obtain the final calving front.}}


\begin{table*}
	\centering
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
		\hline
		\multirow{3}{*}{Score}		& \multirow{3}{*}{\makecell{Tolerance \\ in m}}	& \multicolumn{5}{c|}{Enze Zhang et al.}	& \multicolumn{3}{c|}{Proposed Methods}	\\
		&& Zones	& Front Patches	& \makecell{Front Patches \\ with Dilation}	& Front Resize	& \makecell{Front Resize \\ with Dilation}	& Threshold	& CRF	& \makecell {Second\\U-Net}	\\
		\hline
		\multirow{3}{*}{Dice} 		& 0 	& 0.01768	& 0.16188	& 0.07683	& \bf 0.18137	& 0.17573	& 0.11760 	& 0.14387		&  0.16027		\\
		& 50 	& 0.07556	& 0.31334		& 0.20036	& 0.34409	& \bf 0.34458	& 0.26559 	& 0.30647	& 0.32447 	\\
		& 100 	& 0.12325	& 0.41625		& 0.26782	& 0.47160	& \bf 0.47632	& 0.40432 	& 0.44376	& 0.46289 	\\
		& 150 	& 0.16150	& 0.48761		& 0.31666	& 0.56570	& \bf 0.57567	& 0.52328 	& 0.55444	& 0.57024 	\\
		& 200 	& 0.18379	& 0.52553		& 0.34051	& 0.61651	& 0.62883	& 0.59075 	& 0.61448	& \bf 0.62961 	\\
		& 250 	& 0.20721	& 0.55979		& 0.36278	& 0.66257	& 0.67658	& 0.65288 	& 0.66954	& \bf 0.68353 	\\
		
		\hline
		
		\multirow{3}{*}{IoU} 		& 0 	& 0.00898	& 0.09107	& 0.04102	& \bf 0.10509	& 0.10037	& 0.06421	& 0.07950		& 0.09082 		\\
		& 50 	& 0.04075	& 0.19470		& 0.11916	& 0.20984	& \bf 0.20985	& 0.15547	& 0.18262		& 0.19581	\\
		& 100 	& 0.06998	& 0.27812		& 0.17024	& 0.31271	& \bf 0.31610	& 0.25923	& 0.28909		& 0.30629 	\\
		& 150 	& 0.09459	& 0.34278		& 0.20987	& 0.39950	& \bf 0.40852	& 0.36250	& 0.38928		& 0.40548 	\\
		& 200 	& 0.10977	& 0.38027		& 0.23060	& 0.45177	& 0.46399	& 0.42845 	& 0.44998		& \bf 0.46681 	\\
		& 250 	& 0.12569	& 0.41544		& 0.24990	& 0.50176	& 0.51699	& 0.49321 	& 0.50955		& \bf 0.52598 	\\
		\hline
	\end{tabular}
	\caption{Quantitative evaluation comparing the approach of Zhang et al.~\cite{zhang2019automatically} with our proposed method and the different post processors.}
	\label{tab:quan_ev}
\end{table*}

\begin{figure*}
	\centering
	\begin{minipage}[b]{0.22\linewidth}
		\centering
		\centerline{\includegraphics[width=1\linewidth]{Figures/final/patch_zone/2012-04-05_TSX_10_1.png}}
		\medskip
	\end{minipage}
	%
	\begin{minipage}[b]{0.22\linewidth}
		\centering
		\centerline{\includegraphics[width=1\linewidth]{Figures/final/patch_front/2012-04-05_TSX_10_1.png}}
		\medskip
	\end{minipage}
	%
	\begin{minipage}[b]{0.22\linewidth}
		\centering
		\centerline{\includegraphics[width=1\linewidth]{Figures/final/patch_front_dilate/2012-04-05_TSX_10_1.png}}
		\medskip
	\end{minipage}
	%
	\begin{minipage}[b]{0.22\linewidth}
		\centering
		\centerline{\includegraphics[width=1\linewidth]{Figures/final/enze/2012-04-05_TSX_10_1.png}}
		\medskip
	\end{minipage}

	\begin{minipage}[b]{0.22\linewidth}
		\centering
		\centerline{\includegraphics[width=1\linewidth]{Figures/final/front_dilate/2012-04-05_TSX_10_1.png}}
		\medskip
	\end{minipage}
	%
	\begin{minipage}[b]{0.22\linewidth}
		\centering
		\centerline{\includegraphics[width=1\linewidth]{Figures/final/front/2012-04-05_TSX_10_1.png}}
		\medskip
	\end{minipage}
	\begin{minipage}[b]{0.22\linewidth}
		\centering
		\centerline{\includegraphics[width=1\linewidth]{Figures/final/crf3/2012-04-05_TSX_10_1.png}}
		\medskip
	\end{minipage}
	%
	\begin{minipage}[b]{0.22\linewidth}
		\centering
		\centerline{\includegraphics[width=1\linewidth]{Figures/final/sec_model/bce/2012-04-05_TSX_10_1.png}}
		\medskip
	\end{minipage}


	\centerline{(a)}\medskip


	\begin{minipage}[b]{0.22\linewidth}
		\centering
		\centerline{\includegraphics[width=1\linewidth]{Figures/final/patch_zone/2006-05-06_RSAT_20_3.png}}
		\medskip
	\end{minipage}
	%
	\begin{minipage}[b]{0.22\linewidth}
		\centering
		\centerline{\includegraphics[width=1\linewidth]{Figures/final/patch_front/2006-05-06_RSAT_20_3.png}}
		\medskip
	\end{minipage}
	%
	\begin{minipage}[b]{0.22\linewidth}
		\centering
		\centerline{\includegraphics[width=1\linewidth]{Figures/final/patch_front_dilate/2006-05-06_RSAT_20_3.png}}
		\medskip
	\end{minipage}
	%
	\begin{minipage}[b]{0.22\linewidth}
		\centering
		\centerline{\includegraphics[width=1\linewidth]{Figures/final/enze/2006-05-06_RSAT_20_3.png}}
		\medskip
	\end{minipage}

	\begin{minipage}[b]{0.22\linewidth}
		\centering
		\centerline{\includegraphics[width=1\linewidth]{Figures/final/front_dilate/2006-05-06_RSAT_20_3.png}}
		\medskip
	\end{minipage}
	%
	\begin{minipage}[b]{0.22\linewidth}
		\centering
		\centerline{\includegraphics[width=1\linewidth]{Figures/final/front/2006-05-06_RSAT_20_3.png}}
		\medskip
	\end{minipage}
	%
	\begin{minipage}[b]{0.22\linewidth}
		\centering
		\centerline{\includegraphics[width=1\linewidth]{Figures/final/crf3/2006-05-06_RSAT_20_3.png}}
		\medskip
	\end{minipage}
	%
	\begin{minipage}[b]{0.22\linewidth}
		\centering
		\centerline{\includegraphics[width=1\linewidth]{Figures/final/sec_model/bce/2006-05-06_RSAT_20_3.png}}
		\medskip
	\end{minipage}

	\centerline{(b)}\medskip
	
	\begin{comment} since only two images
	\begin{minipage}[b]{0.30\linewidth}
		\centering
		\centerline{\includegraphics[
			trim=0cm 10cm 0cm 3cm, clip=true,
			width=1\linewidth]{Figures/final/sec_model/bce/2007-10-27_ENVISAT_20_2.png}}
		\centerline{}\medskip
		\medskip
	\end{minipage}
	\end{comment}
	
	\caption{Qualitative outputs of the different approaches: First using the approach proposed by the authors of Zhang et al. from left to right: Zones, Front Patches, Front Patches with Dilation, Front Resize, and Front Resize with Dilation. Then our approach with the different post processors Threshold, CRF, and Second U-Net. The predicted (red) and manual annotated (green) calving front with overlap regions (yellow) are colorized accordingly.} 
	\label{fig:qual_ev}
\end{figure*}


%%%%%%% END NEW	%%%%%%% 


Figure \ref{fig:zhang_vs_thres} shows an example that illustrates the difference in the output of the framework by Zhang et al.~\cite{zhang2019automatically} (a), (b) and the results of our methodology using the Threshold post processor (c), (d). The pictures display the original SAR image, the predicted glacier front (red) and the manual annotated glacier front (green). We also mark overlapping regions of the predicted and labeled mask (yellow). The outputs differ greatly and are presented in more detail in the region of interest (b), (d). 
The model proposed by Zhang et al.~\cite{zhang2019automatically} creates clearly visible artifacts, which are far off and not related to the actual calving front. The predicted glacier front closely trails the manual delineated front. However, the many green areas also show the inconsistency within the prediction. Our proposed methodology using the Threshold approach generates no artifacts. The shape of the predicted calving front is simplified, so that smaller notches in the calving front are not recognized properly. The general course of the glacier front gets continuously and consistently tracked.
%
\begin{figure*}
	\centering
	\begin{tikzpicture}[zoomboxarray, 
		%connect zoomboxes, 
		zoomboxarray columns=2, 
		zoomboxarray rows=1, 
		zoombox paths/.append style={ultra thick}
		]
		\node [image node] { \includegraphics[width=0.45\linewidth]{Figures/final/enze/2006-05-18_PALSAR_20_2.png} };
		\zoombox[color code=orange!70, magnification=3]{0.90,0.83}
		\zoombox[color code=cyan!70, magnification=3]{0.54,0.35}
		%\zoombox{0.15,0.3}
		%\zoombox[magnification=10]{0.86,0.35}
	\end{tikzpicture}
	
	\begin{tikzpicture}[zoomboxarray, 
		%connect zoomboxes, 
		zoomboxarray columns=2, 
		zoomboxarray rows=1, 
		zoombox paths/.append style={ultra thick, orange!75}
		]
		\node [image node] { \includegraphics[width=0.45\linewidth]{Figures/final/front/2006-05-18_PALSAR_20_2.png} };
		\zoombox[color code=orange!70, magnification=3]{0.90,0.83}
		\zoombox[color code=cyan!70, magnification=3]{0.54,0.35}
		%\zoombox{0.15,0.3}
		%\zoombox[magnification=10]{0.86,0.35}
	\end{tikzpicture}
	\caption{Example SAR image showing differences between Zhang et al.~\cite{zhang2019automatically}  (a), (b) and our method using the Threshold post processor (c), (d). The manual annotated (green) and predicted (red) calving front with overlap regions (yellow) are colorized accordingly.}
	\label{fig:zhang_vs_thres}
\end{figure*}

For the quantitative evaluation we use the metrics intersection over union (IoU) and dice coefficient. Both scores are commonly used for semantic image segmentation. Since we try to predict a segmentation mask with a single pixel width, the initial reported scores are low compared to other segmentation tasks, because a small deviation severely affects the results. Such an accuracy can hardly be achieved. We therefore want to allow small differences by introducing a tolerance factor, which defines a distance between predicted and annotated glacier front that we accept. The tolerance is given in meters. We can translate this distance into pixels using the individual spatial resolution of the SAR images. We implement the tolerance using morphological dilation with a structuring element. The structuring element $B$ is a kernel with a specific size $s$, that results from the tolerance value and the spatial resolution of the image. We dilate predicted and annotated calving front and then calculate the segmentation metrics IoU and dice coefficient, which can be seen in Tab. \ref{tab:quan_ev}.

% s ist kernel_size, B is structuring element
\begin{equation}
	\text{dice}_{s}(y_{\text{true}}, y_{\text{pred}}) = \frac{\delta_B(y_{\text{true}}) * \delta_B(y_{\text{pred}}) }{\delta_B(y_{\text{true}}) + \delta_B(y_{\text{pred}})} 
\end{equation}

The scores are evaluated for the tolerances of 0, 50, 100, 150, 200, and 250 meters. We set a wide range of threshold values, since the quality factors ranging from 1 to 4 in our evaluation set allow a maximum deviation of 230 meters for the manual delineated glacier front. As expected, the metric scores increase with higher tolerances, since nearby segmented pixels now also affect the score.

The approach of Zhang et al.~\cite{zhang2019automatically} shows better metric scores when no tolerance is applied, probably resulting from the patch generation process, which allows the images to be fed with original resolution to the segmentation model. However, this pixel accuracy has limited benefits, due to the previously described inaccuracy of the manual delineated glacier fronts.
This initial advantage gets quickly outperformed as the tolerance factor increases.


Looking at the dice score, the post processor CRF and Second U-Net perform on average about 7\% and 11\% better than the Threshold method. The Second U-Net shows the best quantitative results, but also requires the most initial effort, since another whole deep learning model needs to be trained in advance. We only need to set suitable hyper parameters for the Threshold and CRF approach. 


In Figure \ref{fig:qual_ev} we show a set of automatically delineated glacier fronts using our proposed methods. Each picture shows the original SAR image and the predicted glacier front, manual annotated glacier front, and overlapping regions colored respectively in red, green, and yellow as above.
The images on the left, center, and right panel visualize the different outputs of the post processors Threshold, CRF, and Second U-Net. Although the glacier front has no defined shape or appearance and its boundaries are ambiguous, all post processor can consistently predict its general location due to the accurate approximation of the distance maps by the pixel-wise regression model. However, looking closer at the qualitative results reveals clear differences between the methods. The shape and structure of the glacier front generated by the Threshold post processor is often simpler than the other two delineated SAR images. Also the glacier boundaries are not recognized properly. The Second U-Net post processor shows the best qualitative results, since its prediction closely matches the manual annotated calving front which is also consistent with our quantitative evaluation. The CRF approach shows great results at detecting boundaries of the glacier front, which in some cases or not detected by the other approaches (see Fig. \ref{fig:qual_ev}b). The Conditional Random Field probably integrates information given from the additional SAR image input, which is not available to the Threshold and Second U-Net post processor. 
Incorporating this knowledge into Second U-Net approach, by adding the original SAR image to the model input, could further increase its performance.




